Federated Learning of Nonlinear Temporal Dynamics with Graph Attention-based Cross-Client Interpretability

Networks of modern industrial systems are increasingly monitored by distributed sensors, where each system comprises multiple subsystems that generate high-dimensional time-series. These subsystems are often interdependent, making it important to understand how temporal patterns observed at one subsystem relate to those observed across others. This problem is particularly challenging in decentralized settings where raw measurements cannot be shared, and client observations are heterogeneous. Moreover, in practice, each subsystem (client) operates a fixed, proprietary model that cannot be modified or retrained, limiting the applicability of existing approaches. Separately, nonlinear dynamics make cross-client temporal interdependencies difficult to characterize, as they are embedded implicitly within nonlinear state-transition functions. This paper presents a vertical federated learning framework for learning one-step-ahead cross-client temporal interdependencies under these constraints. Each client maps high-dimensional local observations to low-dimensional latent states using a nonlinear state-space model, while a Graph Attention Network (GAT)-based central server learns a state-transition model over the communicated states. Given a candidate graph skeleton, the server learns state-dependent attention coefficients that capture cross-client interactions. We analytically relate the GAT attention coefficients to the Jacobian of the learned state-transition model, yielding a first-order characterization of cross-client interdependencies. We further establish bounded closeness of the learned dynamics and Jacobians to a corresponding centralized oracle. Synthetic experiments validate the theoretical results on controlled systems with known graph skeletons. Experiments on real-world datasets with unknown graph skeletons demonstrate superior federated root cause analysis over baselines.

==> References.tex <==

% \bibitem{Aliakbari2025}
% J. Aliakbari, et al., ``Decoupled Subgraph Federated Learning,'' \textit{arXiv}, arXiv:2402.19163, May 28, 2025. doi: 10.48550/arXiv.2402.19163.

% \bibitem{Chen2020}
% Y. Chen, et al., ``Iterative Deep Graph Learning for Graph Neural Networks: Better and Robust Node Embeddings,'' \textit{arXiv}, arXiv:2006.13009, Oct. 23, 2020. doi: 10.48550/arXiv.2006.13009.

% \bibitem{Franceschi2020}
% L. Franceschi, et al., ``Learning Discrete Structures for Graph Neural Networks,'' \textit{arXiv}, arXiv:1903.11960, Jun. 19, 2020. doi: 10.48550/arXiv.1903.11960.

% \bibitem{Gong2017}
% M. Gong, et al., ``Causal Discovery from Temporally Aggregated Time Series,'' \textit{Proc. Conf. Uncertainty in Artificial Intelligence (UAI)}, vol. 2017, Aug. 2017, p. 269. [Online]. Available: \url{https://www.ncbi.nlm.nih.gov/pmc/articles/PMC5995575/}


% \bibitem{Li2023}
% J. Li, et al., ``TC-GATN: Temporal Causal Graph Attention Networks With Nonlinear Paradigm for Multivariate Time-Series Forecasting in Industrial Processes,'' \textit{IEEE Trans. Ind. Informat.}, vol. 19, no. 6, pp. 7592--7601, 2023. doi: 10.1109/TII.2022.3211330.

% \bibitem{Liao2020}
% R. Liao, et al., ``Efficient Graph Generation with Graph Recurrent Attention Networks,'' \textit{arXiv}, arXiv:1910.00760, Jul. 17, 2020. doi: 10.48550/arXiv.1910.00760.

% \bibitem{Liu2023b}
% J. Liu, et al., ``Causal Graph Attention Network with Disentangled Representations for Complex Systems Fault Detection,'' \textit{Reliab. Eng. Syst. Saf.}, vol. 235, p. 109232, 2023. doi: 10.1016/j.ress.2023.109232.

% \bibitem{Liu2024b}
% R. Liu, et al., ``Causal Intervention Graph Neural Network for Fault Diagnosis of Complex Industrial Processes,'' \textit{Reliab. Eng. Syst. Saf.}, vol. 251, p. 110328, 2024. doi: 10.1016/j.ress.2024.110328.

% \bibitem{Liu2024a}
% Y. Liu and B. Jafarpour, ``Graph Attention Network with Granger Causality Map for Fault Detection and Root Cause Diagnosis,'' \textit{Comput. Chem. Eng.}, vol. 180, p. 108453, 2024. doi: 10.1016/j.compchemeng.2023.108453.

% \bibitem{Ma2023}
% T. Ma, et al., ``Federated Learning of Models Pre-Trained on Different Features with Consensus Graphs,'' \textit{arXiv}, arXiv:2306.01240, Jun. 2, 2023. doi: 10.48550/arXiv.2306.01240.

% \bibitem{Meng2021}
% C. Meng, et al., ``Cross-Node Federated Graph Neural Network for Spatio-Temporal Data Modeling,'' \textit{arXiv}, arXiv:2106.05223, Jun. 9, 2021. doi: 10.48550/arXiv.2106.05223.

% \bibitem{Scarselli2009}
% F. Scarselli, et al., ``The Graph Neural Network Model,'' \textit{IEEE Trans. Neural Netw.}, vol. 20, no. 1, pp. 61--80, 2009. doi: 10.1109/TNN.2008.2005605.

% \bibitem{Velickovic2018}
% P. Veličković, et al., ``Graph Attention Networks,'' \textit{arXiv}, arXiv:1710.10903, Feb. 4, 2018. doi: 10.48550/arXiv.1710.10903.

% \bibitem{Wang2024}
% H. Wang, et al., ``Causal-Trivial Attention Graph Neural Network for Fault Diagnosis of Complex Industrial Processes,'' \textit{IEEE Trans. Ind. Informat.}, vol. 20, no. 2, pp. 1987--1996, 2024. doi: 10.1109/TII.2023.3282979.

% \bibitem{Guo2019}
% K. Guo, Y. Lin, N. Feng, C. Song, and H. Wan,
% ``Adaptive Graph Convolutional Recurrent Network for Traffic Forecasting,''

% \textit{Proc. AAAI Conf. Artificial Intelligence (AAAI)}, vol. 33, no. 1, pp. 922--929, Jul. 2019.
% doi: 10.1609/aaai.v33i01.3301922.

% \bibitem{Wu2022}
% L. Wu, Y. Gao, H. Xu, X. Liu, S. Zheng, and S. Z. Li, ``AutoGCL: Automated Graph Contrastive Learning via Learnable View Generators,'' \textit{Proc. Int. Conf. Learn. Represent. (ICLR)}, 2022. [Online]. Available: \url{https://arxiv.org/abs/2104.07145}

% \bibitem{He2021}
% C. He, et al., ``FedGraphNN: A Federated Learning Benchmark System for Graph Neural Networks,'' \textit{Proc. IEEE/ACM Web Conf. (WWW)}, 2021, pp. 912--922. doi: 10.1145/3442381.3450070.

% \bibitem{Liu2021}
% Liu, Y., et al., ``Federated Graph Neural Network for Privacy-Preserving Node Classification,'' \textit{Proceedings of the AAAI Conference on Artificial Intelligence}, vol. 35, no. 9, pp. 8546--8554, 2021.

% \bibitem{He2021b}
% He, C., et al., ``SpreadGNN: Decentralized Multi-Task Federated Learning for Graph Neural Networks on Graphs with Missing Node Features,'' \textit{Proceedings of the ACM Web Conference (WWW)}, pp. 2828--2837, 2021.

% \bibitem{Zhang2021}
% Zhang, J., et al., ``Federated Learning for Spatio-Temporal Data Mining: A Survey,'' \textit{Proceedings of the 30th ACM International Conference on Information and Knowledge Management (CIKM)}, pp. 4653--4660, 2021.

% \bibitem{Jia2023}
% Y. Jia and C. Zhang, ``Promoting Fairness in GNNs: A Characterization of Stability,'' \textit{arXiv}, arXiv:2309.03648, Dec. 12, 2023. doi: 10.48550/arXiv.2309.03648.


==> old_GrangerCausalityAnalysis.tex <==
In this section, we describe our decentralized framework for root cause discovery in nonlinear dynamical systems. Our goal is to demonstrate that this decentralized approach can converge to the performance of a centralized oracle while also providing interpretable causality analysis. In centralized setting, all measurements are available and can be aggregated and can naturally captures inter-dependencies between clients. However, in decentralized setting, we cannot use all raw measurements directly. Instead, we estimate missing information from other clients through the augmentation mechanism at the client side and the GNN at the server. Thus, we propose that the GNN at the server should mirror the behavior of the centralized oracle.


To show that server-side modeling captures cross-client interdependencies, we take the Jacobian of the GNN model. Intuitively: if a function takes multiple inputs and produces outputs, the Jacobian matrix tells you how much each output changes with respect to each input.
Recall the server model:
\begin{equation}
    (h_t^m)_s =
\sigma\left(
\sum_{n \in \mathcal{N}(m)}
\alpha_{mn}\, W_{mn}\, (\hat{h}_{t-1}^n)_c
\right).
\end{equation}
Each input $(\hat{h}_{t-1}^n)_c$ represents the neighboring nodes' state estimate from the previous timestep, and each output represents the latent state of the server. Then, the Jacobian of this function gives what we need.\\


\subsection{Derivation of the Jacobian Matrix of Server-Side Graph Model}

\begin{assumption}[Known graph structure]
The graph topology is fixed and known \emph{a priori}.
Equivalently, the adjacency matrix \(A \in \{0,1\}^{M\times M}\) is given. For each client/node \(m\), its neighbor set
\(\mathcal{N}(m) := \{\, n \;:\; A_{mn} \neq 0 \,\}\) is known and does not change
during the derivation.
\end{assumption}

\begin{assumption}[Independence of client latent states across nodes]
Client (node) latent states at time \(t\!-\!1\) are independent across nodes in the
sense that the cross-terms vanish and the self-term is the identity:
\begin{equation}
\frac{\partial \,(\hat{h}_{t-1}^n)_c}{\partial \,(\hat{h}_{t-1}^j)_c}
=
\begin{cases}
I_{d_{\mathrm{in}}}, & \text{if } n=j,\\[4pt]
0_{d_{\mathrm{in}}\times d_{\mathrm{in}}}, & \text{if } n\neq j.
\end{cases}
\end{equation}
\end{assumption}

The goal is to compute the Jacobian block with respect to a specific neighbor $j$:
\begin{equation}
          J_{m\leftarrow j} \;:=\; \frac{\partial\, (h_t^m)_s}{\partial\, (\hat{h}_{t-1}^j)_c}
          \;\in\; \mathbb{R}^{d_{\mathrm{out}}\times d_{\mathrm{in}}}.
\end{equation}


Therefore,
new $e$ version:
\begin{equation}
\begin{aligned}
J_{m \leftarrow j}
&= \operatorname{diag}\!\big(\sigma'(s_m)\big) \Bigg[
\sum_{n \in \mathcal{N}(m)}
W_{mn} (\hat{h}^{\,n}_{t-1})_c \cdot
\\[4pt]
&\quad \cdot\;
\frac{
\exp(e_{mn}) \left(
(\delta_{nj} \sum\limits_{r \in \mathcal{N}(m)} \exp(e_{mr}))
- \exp(e_{mj})
\right)
}
{
\left( \sum\limits_{r \in \mathcal{N}(m)} \exp(e_{mr}) \right)^2
}
\\[4pt]
&\quad \cdot\;
\frac{
\partial e_{mj}
}{
\partial (\hat{h}^{\,j}_{t-1})_c
}
+\;
\frac{
\exp(e_{mj})
}{
\sum\limits_{r \in \mathcal{N}(m)} \exp(e_{mr})
}
\cdot W_{mj}
\Bigg].
\end{aligned}
\end{equation}





% old $a$ version:
% \begin{equation}
% \begin{aligned}
% J_{m \leftarrow j}
% &=
% \operatorname{diag}\big(\sigma'(s_m)\big)
% \Bigg[
% \sum_{n\in\mathcal N(m)}
% W_{mn}(\hat h_{t-1}^{\,n})_c\,
% \alpha_{mn}(\delta_{nj} - \alpha_{mj})
% \\[-2pt]
% &\quad\;\;
% \times\;
% \frac{\partial e_{mj}}{\partial (\hat{h}^{\,j}_{t-1})_c}
% +
% \alpha_{mj}\,W_{mj}
% \Bigg].
% \end{aligned}
% \end{equation}
% \endgroup



The Jacobian $J_{m \leftarrow j}$ tells you how node $m$'s update responds to 
perturbations in node $j$'s features. There are two pathways: 
(i) an indirect one via the redistribution of attention among neighbors 
(competition in the softmax), and 
(ii) a direct one via node $j$'s own message. 
Both are modulated by the nonlinearity at node $m$.



